The Impact of Complex and Informed Adversarial Behavior in Graphical Coordination Games

How does system-level information impact the ability of an adversary to degrade performance in a networked control system? How does the complexity of an adversary's strategy affect its ability to degrade performance? This paper focuses on these questions in the context of graphical coordination games where an adversary can influence a given fraction of the agents in the system, and the agents follow log-linear learning, a well-known distributed learning algorithm. Focusing on a class of homogeneous ring graphs of various connectivity, we begin by demonstrating that minimally connected ring graphs are the most susceptible to adversarial influence. We then proceed to characterize how both (i) the sophistication of the attack strategies (static vs dynamic) and (ii) the informational awareness about the network structure can be leveraged by an adversary to degrade system performance. Focusing on the set of adversarial policies that induce stochastically stable states, our findings demonstrate that the relative importance between sophistication and information changes depending on the the influencing power of the adversary. In particular, sophistication far outweighs informational awareness with regards to degrading system-level damage when the adversary's influence power is relatively weak. However, the opposite is true when an adversary's influence power is more substantial.

==> uninformed.tex <==
% !TEX root = main.tex

Here, we provide a proof of Theorem \ref{theorem:SU_opt}, which characterizes the minimal efficiency a static uninformed adversary can induce on a $k$-connected ring graph. The arguments rely on an extension of intermediate step 1 from the proof of Theorem \ref{theorem:SI_opt} to $k$-connected ring graphs. 

In particular, the necessary and sufficient condition to stabilize a $y$-segment in a $k$-connected ring graph is \begin{equation}\label{eq:ystable_kring}
		|S_y \cap L_y| \geq \left\lfloor \alpha\left( k |L_y| + \frac{k(k+1)}{2} \right) \right\rfloor + k(k+1) + 1, 
\end{equation}
and the spacing from two sequential $y$ adversaries within $L_y$ is no more than $\left\lceil \frac{k}{\alpha} \right\rceil$. Note that according to this condition, the segment length must also satisfy $|L_y| \geq k + 1$. 

A derivation of the condition is as follows. There are $\sum_{j=1}^k (|L_y| - j)$ links between  agents in $L_y$. Assuming $|L_y|$ is large enough ($|L_y| \geq k+1$), there are $2\sum_{j=1}^k j$ links from $L_y$ to outside $L_y$. The potential of $y^{L_y}$ (all agents in $L_y$ play $y$) exceeds that of $x^{L_y}$ (all play $x$) if
\begin{equation}
	|S_y \cap L_y| + \sum_{j=1}^k (|L_y| - j) > (1+\alpha)\left[ \sum_{j=1}^k (|L_y| - j) + 2\sum_{j=1}^k j \right]
\end{equation}
which reduces to \eqref{eq:ystable_kring}. One can prove sufficiency in a similar manner as step 1 from the previous section -- by allocating the $y$-adversaries with a spacing of $\left\lceil \frac{k}{\alpha} \right\rceil$ apart, the potential of $y^{L_y}$ exceeds that of any other $a^{L_y} \neq \{y^{L_y},x^{L_y} \}$. We omit these details for space concerns.

We are now ready to prove Theorem \ref{theorem:SU_opt}.
    A static and uninformed policy cannot strategically place adversarial nodes in the network. It can only specify the numbers of $x$ and $y$ adversaries. Its baseline performance is given by the minimal damage that can be inflicted over all possible allocations of these adversaries. Hence to characterize \eqref{eq:SU_OPT},  we seek the allocation of adversaries that ensures the best-case efficiency for the network.
    
     
    
    
    
    
    First, we consider the case $\gamma < k\alpha$. The adversarial nodes can be allocated sparsely enough across the entire network such that the condition \eqref{eq:ystable_kring} is violated. Consequently, the all $x$ profile is the unique stochastically stable state. Therefore, no damage can be inflicted on the system in this regime. Note that if $k\alpha > 1$, no damage is possible regardless of the adversary's budget.
    
    Now, consider $\gamma > k\alpha$. If $k\alpha < 1$ and $G \in \mcal{G}^k$ is sufficiently large, an allocation of $y$-adversaries according to \ref{eq:ystable_kring} would ensure conversion of the entire network to $y$, giving an efficiency of $\frac{1}{1+\alpha}$. However, let us consider a  re-allocation of these adversaries that maximally mitigates such damage. The idea is to  only allow a minimal fraction $f$ of the network to be converted to $y$, while the rest of the network can stay at $x$. 
    
    Suppose $y$-adversaries are allocated to every agent in a contiguous segment, whose length is a fraction $f$ of the entire network. Suppose this segment is sufficiently long such that \eqref{eq:ystable_kring} is satisfied. Now, the remaining adversaries $\gamma - f$ should be allocated to the rest of the network such that the remaining fraction $1-f$ of the network is still stable to $x$. An adversarial agent density of up to $k\alpha$ in the remaining network nullifies their effects. The smallest $f$ that satisfies these conditions is given by $f = \frac{\gamma - k\alpha}{1 - k\alpha}$. This establishes \eqref{eq:SU_OPT}. Note in this analysis, the adversary exclusively chooses to implement $y$-adversaries. Based on the above arguments, an optimal static uninformed policy never chooses to use $x$-adversaries.


% We extend the necessary and sufficient condition \eqref{eq:y_nec} on the number of adversarial nodes required for $y$-segments to $k$-connected ring graphs.
%
% \begin{lemma}\label{lem:ysegk}
%     Let $G \in \mcal{G}^k$ for $k \in \{1,2,\ldots,n/2\}$ and let $S$ be an allocation of adversarial agents. A $y$ segment $L_y$ appears in the unique stochastically stable state if and only if  
%     \begin{equation}\label{eq:ystable_cond1}
% 		\alpha < \frac{|S_y \cap L_y| - k(k+1)}{k |L_y| + \frac{k(k+1)}{2}}.
% 	\end{equation}
% 	and the spacing from two sequential $y$ adversaries within $L_y$ is no more than $\left\lceil \frac{k}{\alpha} \right\rceil$. Note the segment length must also satisfy $|L_y| \geq k + 1$.
% \end{lemma}
% %
% \begin{proof}
% 	There are $\sum_{j=1}^k (|L_y| - j)$ links between  agents in $L_y$. Assuming $|L_y|$ is large enough ($|L_y| \geq k+1$), there are $2\sum_{j=1}^k j$ links from $L_y$ to outside $L_y$. The potential of $y^{L_y}$ (all agents in $L_y$ play $y$) exceeds that of $x^{L_y}$ (all play $x$) if
% 	\begin{equation}
% 		|S_y \cap L_y| + \sum_{j=1}^k (|L_y| - j) > (1+\alpha)\left[ \sum_{j=1}^k (|L_y| - j) + 2\sum_{j=1}^k j \right]
% 	\end{equation}
% 	which reduces to \eqref{eq:ystable_cond1}.
% \end{proof}
% The following Lemma establishes how sparse $y$ adversarial nodes can be allocated along a segment such that no agents are converted to $y$ in the stochastically stable state of a $k$-connected ring graph.
% %
% \begin{lemma}\label{lem:spread}
% 	Let $L = \{j,\ldots,j+|L|-1\}$ be any contiguous segment of $G \in \mcal{G}^k$. For any fraction $f < k\alpha$, consider the set of indices
% 	\begin{equation}\label{eq:placements}
% 		I = \left\{i \in L : \left\lfloor f (|L|-i+1) \right\rfloor - \left\lfloor f (|L|-i) \right\rfloor > 0 \right\}.
% 	\end{equation}
% 	In words, $I$ selects one every $f^{-1}$ agent in $L$. Suppose $S_y \cap L = I$. Then we have $a_i = x$, $\forall i \in L$ in the stochastically stable state $a$.
% \end{lemma}
% %
% \begin{proof}
% 	Due to $f < k\alpha$, the adversary spacing condition of Lemma \ref{lem:ysegk} is not met. In order for any $y$ segment within $L$ to be stabilizable, the conditions \eqref{eq:type1_condition} and \eqref{eq:type2_condition} must be met. However, the adversary placements specified by \eqref{eq:placements} ensures these conditions are never met.
% \end{proof}
% %


% We are now in a position to prove the first part of Theorem \ref{thm:uninformed}, equation \eqref{eq:SU_OPT}. This describes the fundamental lower bound on a static uninformed policy $\pi \in \Pi$ over any graph $G \in \mcal{G}^k$. 


